Better Adherence, Richer Context: A Field Evaluation of LLM-Powered Conversational Voice Diaries for Sleep

Sleep diaries are central to behavioral sleep medicine and cognitive behavioral therapy for insomnia, yet daily completion is difficult to sustain, and static forms often provide limited context for interpreting night-to-night sleep variation. We designed an LLM-powered conversational voice diary that delivers clinically grounded morning and evening sleep diary questions through proactive smart-speaker prompts, structured conversational intake, and adaptive follow-up dialogue. We evaluated the system in a four-week between-subjects field study with 30 university students, comparing it with a text-based mobile diary using matched diary items, reporting windows, and reminder intervals. Compared with the text-based diary, the conversational voice diary showed higher adherence and elicited more detailed contextual self-report about routines, stressors, environmental conditions, and other sleep-related factors. Participants also described the voice diary as easier to integrate into daily routines, despite longer perceived completion time. However, voice-based conversational intake produced lower completeness for some structured diary fields, revealing a trade-off between expressive richness and structured precision. These findings show both the promise and the challenge of using LLM-powered conversational voice assistants for longitudinal health self-report.

==> comments.tex <==
\begin{enumerate}
    \item Number of tokens: total count of tokens (words) in the segment after simple tokenization.
    \item Percentage lexical density: Percentage of tokens that are content words (nouns, verbs, adjectives, adverbs). Spoken forms tend to have lexical densities below 40\% \cite{castello2008text}. 

    \item Number of words in noun-phrases: Total number of tokens that belong to any spaCy‐detected noun phrase.

    \item Shannon entropy bits:  The average information content per token was computed based on the segment’s token–frequency distribution. 
    %In English, Shannon’s estimate of $0.6$–$1.3$ bits per character corresponds to approximately $2.7$–$5.8$ bits per word (to be double checked). 
    This serves as a proxy for informativeness, as mentioned in \cite{xiao2020tell}.


    \item Cross entropy bits: Average GPT-2 surprisal (in bits) per token, indicating how unpredictable the phrasing is.

    \item Type–Token Ratio (TTR): Ratio of unique tokens to total tokens, measuring raw lexical diversity.

    \item Moving‐Average TTR: Length‐adjusted lexical diversity computed as the average TTR over sliding windows. (less sensitive to length of text). 
    
    \item Average word length: Mean number of characters per token, reflecting lexical sophistication.
 
    \item Proposition density: The approximate number of proposition markers (finite verbs or clausal dependencies) was computed per 10 words
    \item Max tree depth:  Maximum depth of the dependency parse tree across the segment’s sentences.
    
    \item CPIDR score: Approximated CPIDR idea density (propositions per ten words) based on finite verbs and clausal dependencies.
\end{enumerate}


  \item \textbf{Number of tokens:} Total count of tokens (words) in the segment after basic tokenization. We included numbers in tokens to account for time and durations. 
    
    \item \textbf{Lexical density (\%):} Proportion of tokens that are content words (nouns, verbs, adjectives, adverbs). 
    Spoken responses typically exhibit lexical densities below 40\% \cite{castello2008text}.
    
    \item \textbf{Words in noun phrases:} Total number of tokens belonging to any spaCy‐detected noun phrase.
    
    \item \textbf{Shannon entropy (bits):} Average information content per token, computed from the segment’s token–frequency distribution. 
    Used as a proxy for informativeness \cite{xiao2020tell}.
    %In English, Shannon’s estimate of $0.6$–$1.3$ bits per character corresponds to approximately $2.7$–$5.8$ bits per word (to be double checked). 
    
    \item \textbf{Cross entropy (bits):} Average GPT-2 surprisal (in bits) per token, reflecting the unpredictability of phrasing.
    
    \item \textbf{Type–Token Ratio (TTR):} Ratio of unique tokens to total tokens, measuring lexical diversity.
    
    \item \textbf{Moving‐average TTR:} Length‐adjusted lexical diversity, computed as the average TTR over sliding windows; less sensitive to text length.
    
    \item \textbf{Average word length:} Mean number of characters per token, reflecting lexical sophistication.
    
    \item \textbf{Proposition density:} Approximate number of proposition markers (finite verbs or clausal dependencies) per 10 words.
    
    \item \textbf{Maximum tree depth:} Maximum depth of the dependency parse tree across the segment’s sentences.
    
    \item \textbf{CPIDR score:} Approximated CPIDR idea density (propositions per 10 words) based on finite verbs and clausal dependencies.


    \begin{enumerate}
    \item Number of tokens: VA $>$ Text; $p < .001$
    \item Percentage lexical density: Text $>$ VA; $p < .001$ \\
    (because speech has more fillers compared to rigid text answers.)
    \item Number of words in noun-phrases: VA $>$ Text; $p < .001$
    \item Shannon entropy bits: VA $>$ Text; $p < .001$
    \item Cross entropy bits: Text $>$ VA; $p < .001$
    \item TTR: Text $>$ VA; $p = .002$
    \item Average word: VA $>$ Text; $p < .001$
    \item Proposition density: VA $>$ Text; $p < .001$
    \item Max tree depth: VA $>$ Text; $p < .001$
    \item CPIDR score: VA $>$ Text; $p < .001$
\end{enumerate}
